VeriGen: A Large Language Model for Verilog Code Generation

In this study, we explore the capability of Large Language Models (LLMs) to automate hardware design by generating high-quality Verilog code, a common language for designing and modeling digital systems. We fine-tune pre-existing LLMs on Verilog datasets compiled from GitHub and Verilog textbooks. We evaluate the functional correctness of the generated Verilog code using a specially designed test suite, featuring a custom problem set and testing benches. Here, our fine-tuned open-source CodeGen-16B model outperforms the commercial state-of-the-art GPT-3.5-turbo model with a 1.1% overall increase. Upon testing with a more diverse and complex problem set, we find that the fine-tuned model shows competitive performance against state-of-the-art gpt-3.5-turbo, excelling in certain scenarios. Notably, it demonstrates a 41% improvement in generating syntactically correct Verilog code across various problem categories compared to its pre-trained counterpart, highlighting the potential of smaller, in-house LLMs in hardware design automation.

==> section/08Conclusions.tex <==

\section{Conclusions}
This paper describes a new paradigm for automatically generating and verifying Verilog from \acp{LLM}. 
Using the presented Pass@(\textit{scenario}*$n$) values from Tables~\ref{tbl:compiled}-\ref{tbl:results}, pre-tuned LLMs produced completions that are functionally correct only $1.09\%$ of the time. This number increases to $27.0\%$ after tuning, showing a clear benefit to fine-tuning \acp{LLM} over a specific language.
 The fine-tuned CodeGen-16B LLM was the most successful in completions with respect to functional correctness.
Overall it produced functionally correct code $41.9\%$ of time, whereas the commercially available state-of-the-art (non-fine-tuned) GPT-3.5-turbo and GPT4 produced functionally correct code $43.1\%$ and XX\% of time. 
%This is impressive for CodeGen-16B as it is estimated to be about 11 times smaller in terms of number of parameters. We hypothesize that fine tuning Code-davinci-002 would produce even better results.
%Future work could examine applications of the generated code.

%Future Work - BG (Feel free to edit)
% A direction for future work is to judge how secure the generate Verilog code is. Prior effort \citep{pearce_asleep_2022} was conducted over pre-tuned LLMs. It would be interesting to compare those results with fine-tuned LLMs

\label{sec:conclusions}

\section*{Acknowledgements}

This research work was supported in part by NSF Award 1553419, NSF Award 1646671, NSF Award 2039607, and ARO Award 77191NC. The opinions, findings, and conclusions, or recommendations expressed are those of the author(s) and do not necessarily reflect the views of any sponsors.

% # 2039607


==> section/preamble/preamblelistingsconf.tex <==
\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\makeatletter
\let\old@lstKV@SwitchCases\lstKV@SwitchCases
\def\lstKV@SwitchCases#1#2#3{}
\makeatother
\usepackage{lstlinebgrd}
\makeatletter
\let\lstKV@SwitchCases\old@lstKV@SwitchCases

\lst@Key{numbers}{none}{%
    \def\lst@PlaceNumber{\lst@linebgrd}%
    \lstKV@SwitchCases{#1}%
    {none:\\%
     left:\def\lst@PlaceNumber{\llap{\normalfont
                \lst@numberstyle{\thelstnumber}\kern\lst@numbersep}\lst@linebgrd}\\%
     right:\def\lst@PlaceNumber{\rlap{\normalfont
                \kern\linewidth \kern\lst@numbersep
                \lst@numberstyle{\thelstnumber}}\lst@linebgrd}%
    }{\PackageError{Listings}{Numbers #1 unknown}\@ehc}}
\makeatother



\usepackage{lstlinebgrd} % see http://www.ctan.org/pkg/lstaddons




% \lstset{ 
% %   escapeinside={(*@}{@*)},
%   backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
%   basicstyle=\normalsize,        % the size of the fonts that are used for the code
% %   breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
%   breaklines=true,                 % sets automatic line breaking
% %   captionpos=b,                    % sets the caption-position to bottom
%   commentstyle=\color{mygreen},    % comment style
% %   deletekeywords={...},            % if you want to delete keywords from the given language
% %   escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
% %   extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
%   frame=single,	                   % adds a frame around the code
% %   keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
%   keywordstyle=\color{blue},       % keyword style
%   language=C,                 % the language of the code
% %   morekeywords={*,...},            % if you want to add more keywords to the set
%   numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
%   numbersep=5pt,                   % how far the line-numbers are from the code
%   numberstyle=\tiny\color{black}, % the style that is used for the line-numbers
% %   rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
% %   showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
% %   showstringspaces=false,          % underline spaces within strings only
% %   showtabs=false,                  % show tabs within strings adding particular underscores
% %   stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
%   stringstyle=\color{mymauve},     % string literal style
% %   tabsize=2,	                   % sets default tabsize to 2 spaces
% %   title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
% %   %framesep=0pt,framerule=0pt,
% %   %aboveskip=0pt,belowskip=0pt
% }



\global\setlength{\fboxsep}{0pt}
%\global\setlength{\textwidth}{474.18663pt}


\tcbset{
  aibox/.style={
    width=435.18663pt,
    top=10pt,
    colback=white,
    colframe=black,
    colbacktitle=black,
    enhanced,
    center,
    attach boxed title to top left={yshift=-0.1in,xshift=0.15in},
    boxed title style={boxrule=0pt,colframe=white,},
  }
}
\newtcolorbox{AIbox}[2][]{aibox,#1}
\definecolor{britishracinggreen}{rgb}{0.0, 0.44, 0.0}
\definecolor{aigold}{RGB}{244,210, 1} 
\definecolor{aigreen}{RGB}{210,244,211} 
\newcommand{\lightgreen}[1]{\fcolorbox{aigreen}{aigreen}{\parbox{\linewidth}{#1}}}
\sethlcolor{aigreen}

\definecolor{aired}{RGB}{255,180,181} 
\newcommand{\lightred}[1]{\colorbox{aired}{\parbox{\linewidth}{#1}}}


\newtcbox{\mybox}[1][green]{on line,
arc=0pt,outer arc=0pt,colback=#1!10!white,colframe=#1!50!black,
boxsep=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,
boxrule=0pt,bottomrule=0pt,toprule=0pt}

% \usemintedstyle{vs}
% \newcommand{\mscomment}[1]{\textcolor{blue}{\textbf{[#1 --Seb]}}}
\newcommand{\DVcom}[1]{\textcolor{red}{[DV3: #1]}}
\newcommand{\yintat}[1]{\textcolor{red}{[YinTat: #1]}}
\newcommand{\varun}[1]{\textcolor{red}{[VC: #1]}}
\newcommand{\hamid}[1]{\textcolor{red}{[HP: #1]}}
\newcommand{\ronen}[1]{\textcolor{red}{[RE: #1]}}
\newcommand{\johannes}[1]{\textcolor{red}{[JG: #1]}}
\newcommand{\DV}{GPT-4\xspace}
\usepackage{listings}
% \lstset{basicstyle=\ttfamily, columns=flexible, breaklines=true, mathescape=true}

% \lstdefinestyle{mystyle}{
%     backgroundcolor=\color{white},
%     commentstyle=\color{britishracinggreen},
%     keywordstyle=\color{blue},
%     numberstyle=\tiny\color{black},
%     stringstyle=\color{purple},
%     basicstyle=\ttfamily\footnotesize,
%     breakatwhitespace=false,
%     breaklines=true,
%     keepspaces=true,
%     numbers=left,
%     numbersep=5pt,
%     showspaces=false,
%     showstringspaces=false,
%     showtabs=false,
%     tabsize=2,
%     frame=none  % Add this line
% }

\usepackage{xcolor}

\lstdefinelanguage{verilog}{
  keywords={module, endmodule, input, output, wire, reg, assign, always, begin, end, posedge},
  keywordstyle=\color{blue}\bfseries,
  stringstyle=\color{mymauve},
  commentstyle=\color{mygreen},
  morecomment=[l]//,  % Line-based comments
  morecomment=[s]{/*}{*/},  % Block-based comments
}


\lstset{
  language=verilog,
  basicstyle=\scriptsize\ttfamily\linespread{0.0001},
  numbers=left,
  numberstyle=\tiny\color{gray},
  numbersep=5pt,
  breaklines=true,
  breakatwhitespace=true,
  tabsize=3,
  xleftmargin=0.000001in,  % Adjust this value to move the numbers closer to or further from the left margin
  columns=fullflexible,
}
